"In Dialogues We Learn": Towards Personalized Dialogue Without Pre-defined Profiles through In-Dialogue Learning

Personalized dialogue systems have gained significant attention in recent years for their ability to generate responses in alignment with different personas. However, most existing approaches rely on pre-defined personal profiles, which are not only time-consuming and labor-intensive to create but also lack flexibility. We propose In-Dialogue Learning (IDL), a fine-tuning framework that enhances the ability of pre-trained large language models to leverage dialogue history to characterize persona for completing personalized dialogue generation tasks without pre-defined profiles. Our experiments on three datasets demonstrate that IDL brings substantial improvements, with BLEU and ROUGE scores increasing by up to 200% and 247%, respectively. Additionally, the results of human evaluations further validate the efficacy of our proposed method.

==> discussion.tex <==
\subsection{Case Study}

\begin{figure}[]
\centerline{\includegraphics[width=0.5\textwidth]{image/case_study.pdf}}
\caption{A case study. Keywords in the profile are marked in red, while the corresponding keywords that have high attention weight within dialogue sessions are bolded and highlighted with a yellow background.}
\label{fig:case_study}
\end{figure}

To investigate the specific content within dialogue sessions that a model trained with IDL focuses on when crafting responses, we conducted an analysis of the attention weights during the reply generation process, as illustrated in Figure~\ref{fig:case_study}. We identified the top 100 tokens receiving the highest attention weights within the dialogue sessions and examined their correspondence with the personality-related keywords found in the established golden profile. The experimental findings indicate that the LLaMA2-13B model, prior to IDL training, typically concentrates on an average of 9 keywords. However, the same model, once trained with IDL, shows an enhanced focus on 13 keywords. This improvement suggests that IDL training significantly enhances the model's ability to accurately leverage persona information during dialogue exchanges.

\subsection{Effect of Dialogue Sessions}

\begin{figure}[]
\centerline{\includegraphics[width=0.5\textwidth]{image/sessions.pdf}}
\caption{Experiments with the different dialogue sessions on the Movie and LIGHT dataset.}
\label{fig:sessions}
\end{figure}

In IDL, the model learns personality-related information from the dialogue sessions and generates corresponding responses. Intuitively, the number of dialogue sessions influence the quality of replies. We conduct experiments on the datasets Movie and LIGHT and report this influence in Figure~\ref{fig:sessions}. The figure illustrates that with an increase in the number of dialogue sessions, there is a general improvement in the quality of responses. This indicates that engaging in dialogue contributes positively to generating responses related to the persona. However, the improvement is not consistent, and adding more dialogue sessions does not automatically lead to better quality responses. This inconsistency can be attributed to the variation in persona information across different sessions, which complicates the extraction of targeted persona information.

==> table2_ft.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[t!]
\small
\centering
\begin{tabular}{cclccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Size} & \multirow{2}{*}{Model} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Coherence} & \multicolumn{2}{c}{Diversity} & \multicolumn{2}{c}{Persona} \\ \cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10} 
 &  &  &  & BLEU-1 & ROUGE-L & Dist-1 & Dist-2 & P-F1 & P-Co \\ \midrule
\multirow{7}{*}{Movie} & \multirow{3}{*}{7B} 
 & Vicuna & FT & {\ul 28.72} & 10.99 & {\ul 89.17} & 93.14 & 13.99 & 21.75 \\					
 &  & LLaMA-2 & FT & 6.12 & {\ul 5.95} & 65.38 & {\ul 91.10} & {\ul 11.70} & {\ul 18.95} \\
 &  & LLaMA-2 & IDL & \textbf{26.08}$^\dag$ & \textbf{10.92}$^\dag$ & \textbf{91.73}$^\dag$ & \textbf{93.32}$^\dag$ & \textbf{19.14}$^\dag$ & \textbf{22.35}$^\dag$ \\ 
 \cmidrule(lr){2-10}
 & \multirow{4}{*}{13B} 
 & Vicuna & FT & 27.22 & 11.02 & 86.13 & 90.42 & 14.94 & 23.38 \\	
 &  & WizardLM & FT & {\ul 26.23} & {\ul 11.63} & {\ul 97.17} & {\ul 98.98} & {\ul 13.74} & {\ul 22.86} \\			
 &  & LLaMA-2 & FT & 15.04 & 8.21 & 75.26 & 94.55 & 14.38 & 20.71 \\
 &  & LLaMA-2 & IDL & \textbf{29.17}$^\dag$ & \textbf{13.1} & \textbf{92.65}$^\dag$ & \textbf{94.89}$^\dag$ & \textbf{20.32} & \textbf{24.52} \\ \midrule
\multirow{7}{*}{LIGHT} & \multirow{3}{*}{7B}
 & Vicuna & FT & {\ul 31.14} & {\ul 9.87} & {\ul 83.74} & 89.57 & 14.73 & 22.21 \\	
 &  & LLaMA-2 & FT & 15.41 & 9.88 & 67.74 & {\ul 93.24} & {\ul 16.78} & \textbf{31.99} \\
 &  & LLaMA-2 & IDL & \textbf{29.85}$^\dag$ & \textbf{10.92}$^\dag$ & \textbf{88.03}$^\dag$ & \textbf{93.49}$^\dag$ & \textbf{18.2}$^\dag$ & {\ul 23.04}$^\dag$ \\ 
 \cmidrule(lr){2-10}
 & \multirow{4}{*}{13B} 
 & Vicuna & FT & 25.75 & 8.16 & 74.59 & 75.44 & 12.08 & 18.76 \\	
 &  & WizardLM & FT & {\ul 27.1} & {\ul 11.75} & {\ul 94.21} & {\ul 98.67} & {\ul 14.3} & 23.63 \\	
 &  & LLaMA-2 & FT & 24.31 & 10.55 & 75.07 & 96.24 & 17.69 & \textbf{31.48} \\
 &  & LLaMA-2 & IDL & \textbf{29.54}$^\dag$ & \textbf{11.82} & \textbf{90.55}$^\dag$ & \textbf{95.78} & \textbf{16.41} & {\ul 24.79} \\ \bottomrule
\end{tabular}
\caption{Automatic evalution compared to pre-trained large language models on Movie and LIGHT. The best results are in \textbf{bold} and the second best results are \underline{underlined}. ``$\dag$'' indicates that our model passed
the t-test with $p$-value $< 0.05$ in comparison to the best baseline.}
\label{table: table2}
\end{table*}
